Measuring CDNs susceptible to Domain Fronting

Domain fronting is a network communication technique that involves leveraging (or abusing) content delivery networks (CDNs) to disguise the final destination of network packets by presenting them as if they were intended for a different domain than their actual endpoint. This technique can be used for both benign and malicious purposes, such as circumventing censorship or hiding malware-related communications from network security systems. Since domain fronting has been known for a few years, some popular CDN providers have implemented traffic filtering approaches to curb its use at their CDN infrastructure. However, it remains unclear to what extent domain fronting has been mitigated. To better understand whether domain fronting can still be effectively used, we propose a systematic approach to discover CDNs that are still prone to domain fronting. To this end, we leverage passive and active DNS traffic analysis to pinpoint domain names served by CDNs and build an automated tool that can be used to discover CDNs that allow domain fronting in their infrastructure. Our results reveal that domain fronting is feasible in 22 out of 30 CDNs that we tested, including some major CDN providers like Akamai and Fastly. This indicates that domain fronting remains widely available and can be easily abused for malicious purposes.

==> ehical_considerations.tex <==
\section*{Appendix}

\section{Ethics}

For conducting automated tests for domain fronting, we have taken the following measures to strictly adhere to ethical considerations to ensure responsible research practices. Firstly, we do not host any malicious content on any of the tested CDNs. We just make simple requests to already existing customers of the CDNs, aiming to assess potential vulnerabilities rather than engaging in any harmful activities. To avoid any disruption to the CDNs' services, we limited the number of requests sent per CDN to a maximum of 4000. While analyzing DNS traffic, we do not use any Personally Identifiable Information such as IP address and we obtained the necessary IRB approval from involved organizations to access DNS traffic. Throughout the process of parsing DNS logs, we ensured that the privacy of users was protected, and their personal information remained confidential as we were only interested in the domain names and their aliases. By considering these ethical considerations, we ensured that our measurement and analysis of domain fronting were conducted in a responsible and respectful manner. We maintained user privacy, minimized disruptions to CDNs, and used data in a responsible and appropriate manner throughout our research.


\section{CDN Domain Discovery Example}
Consider the following example to understand the steps involved in Domain Discovery. As a concrete example, let $c$ be {\tt edgekey.net}. In this case, we use DNS analysis to collect subdomains of $c$ such as {\tt www.microsoft.com-c-3 .edgekey.net}. To obtain the corresponding domain related to the website hosted by the CDN, we inspect the DNS response that included the CNAME $s.c$ and extract the query name $q$ from the question section of the DNS response where the CNAME was found. By repeating this search for every CDN domain $c \in L_C$, we derive the list $D_C$ of all domains related to websites served by CDN $C$.


\section{Additional Domain Analysis Results}

\noindent \textbf{Popular Domains in CDNs:} CDNs hosting popular domains play a crucial role in facilitating successful domain fronting attacks, primarily due to their lower probability of being blocked by network security tools. When a popular domain is hosted by a CDN, there is a higher chance that the CDN's IP address will be permitted by network security measures, even if a different domain is being requested. This advantageous situation enables attackers to leverage domain fronting as a means to mask their traffic and evade detection more effortlessly. Moreover, CDNs hosting popular domains often possess ample resources to handle substantial volumes of traffic, rendering them an attractive target for malicious actors. Figure~\ref{fig:cdn_domain_counts} also showcases the count of domains that are popular(rankings of {$<=$100k}), per each CDN. Remarkably, in case of {\em 29} CDNs, popular domains accounted for a substantial percentage of 30\%(at least) of the total domains and {\em 34} CDNs were found to host one or more popular domains. This observation signifies that even less renowned CDNs are preferred by popular websites as hosting platforms for their content, despite well-known CDNs like Cloudfront hosting 37\% of the overall encountered domains. 

\subsubsection{CDN and Domain Attribution Reliability}
To establish the reliability of our domain-to-CDN mappings, we conducted an experiment on DNS logs spanning multiple days. Our objective was to examine whether specific domains were consistently associated with a single CDN. The findings revealed that {99.64}\% of the domains consistently mapped to a single CDN, ensuring a stable relationship. As for the remaining domains that was associated with different CDNs across multiple days, it may be so because of using Multi-CDN services~\cite{cui2018multi}, that resolves a domain to different CDNs based on various metrics such as performance overhead, proximity, and other relevant factors. 
% Considering that such cases were negligible small, we continued with our tests after discarding these domains from our dataset.

\noindent \textbf{Malicious Domains in CDNs: } To understand how CDNs are targeted by attackers for performing malicious activities, we track the percentage of malicious actors based on domain check against VT as discussed in system overview. By flagging domains found malicious by at least two security vendors from the list of vendors provided by Virus Total, we found that {\em 11} of the CDNs contained malicious domains as shown in Figure~\ref{fig:cdn_domain_counts} and {\em 27} CDNs contained one or more malicious domains flagged by at least one security vendor. 
% This only serves as the lower bound since the DNS traffic that we analyzed through our academic network already employ measures to detect and block malicious traffic. 


\section{Domain Fronting Process}
The process of domain fronting involves several steps, as depicted in Figure~\ref{fig:dom_fronting}(in Appendix). This involves selecting a legitimate website (e.g., {\tt legitsite.com}) as the SNI, while specifying the actual target site owned by the attacker (e.g., {\tt evilsite.com}) as the {\tt Host} parameter in the HTTP header. (Step 1) Malware running on the victim host issues a DNS query for a legitimate domain name {\tt legitsite.com} served by the abused CDN. (Step 2) The DNS query being for a legitimate domain evades DNS-based malware defenses and returns the IP address of a CDN edge server. Subsequently, (Step 3) the malware connects to the CDN edge server and establishes a TLS session using {\tt legitsite.com} as the SNI but expressing {\tt evilsite.com} as the {\tt Host} in the HTTP request header. Upon reaching the CDN server, the web request is processed based on the information provided in the {\tt Host} header, in this case {\tt evilsite.com}. If content is not cached at the edge server, (Step 4) the CDN forwards the request to the attacker's origin server, obtains a response, and forwards the response back to the victim. 

\begin{figure}[!ht]
    \centering
    \setlength\belowcaptionskip{-1\baselineskip}
    \includegraphics[width=0.85\columnwidth]{figs/dom_fronting_arch.pdf}
    % \addtolength{\belowcaptionskip}{5pt}
    \caption{Domain Fronting Overview}
    \label{fig:dom_fronting}
\end{figure}

\pagebreak

\section{Additional Figures}
<<<<<<< HEAD
=======



>>>>>>> origin/main

\input{tables/cdn_counts}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\columnwidth]{figs/error_code_distribution.pdf}
    \addtolength{\belowcaptionskip}{-5pt}
    \caption{Domain Count per Error code for failed tests}
    \label{fig:error_codes}
\end{figure}


==> mitigations.tex <==
\section{Mitigation Strategies}
Various mitigation strategies have been proposed to detect and block domain fronting. We discuss each of these approaches in detail.

\subsection{Machine Learning}

One approach to mitigating the risks associated with domain fronting involves using machine learning algorithms to analyze network traffic and identify patterns that may indicate the use of domain fronting. This approach can be effective in identifying suspicious traffic, but it can also have limitations and potential drawbacks, such as false positives or the blocking of legitimate traffic.

Machine learning algorithms work by analyzing large amounts of data to identify patterns and make predictions. In the case of domain fronting, machine learning algorithms can be trained to recognize patterns in network traffic that are indicative of domain fronting. For example, the algorithms may be able to identify traffic that uses the same IP address for both the front domain and the back domain, or traffic that has unusual patterns of encryption.

While machine learning algorithms can be effective in detecting domain fronting, they can also have limitations. For example, they may generate false positives, identifying legitimate traffic as suspicious. In addition, attackers may be able to evade detection by using more sophisticated techniques or by modifying their traffic to avoid detection.

\subsection{Deep Packet Inspection}

Another approach to mitigating the risks associated with domain fronting involves using deep packet inspection to examine the contents of network traffic and identify any suspicious activity. This approach can be more accurate than machine learning algorithms, but it can also be more resource-intensive and may require more specialized knowledge and expertise.

Deep packet inspection involves examining the contents of network traffic at a granular level, including the headers and payloads of individual packets. This allows security teams to identify suspicious activity, such as traffic that is encrypted using different algorithms or that has unusual patterns of traffic flow.

While deep packet inspection can be more accurate than machine learning algorithms, it can also be more resource-intensive and may require more specialized knowledge and expertise. In addition, attackers may be able to evade detection by using more sophisticated techniques or by modifying their traffic to avoid detection.

\subsection{Network-Level Blocking}

Finally, some countries have implemented measures to block domain fronting altogether. For example, Russia has blocked access to Telegram, a messaging app that had been using domain fronting to circumvent government censorship. Other countries, such as Iran and China, have also taken steps to restrict the use of domain fronting.

Network-level blocking involves blocking traffic to specific domains or IP addresses based on predefined criteria. This approach can be effective in preventing domain fronting, but it can also be difficult to implement and may have unintended consequences, such as the blocking of legitimate traffic.

Overall, while there are various mitigation strategies available for domain fronting, each approach has its own strengths and weaknesses. It is important for security teams to carefully evaluate their options and choose the approach or combination of approaches that is most appropriate for their specific needs and circumstances.

==> tables/dns_cname.tex <==
\begin{table}[htbp]
    \begin{center}
        \captionof{table}{Examples of DNS CNAME record}
        \label{tab:dns_cname_record}
        \scriptsize
        \begin{tabular}{c|c|c}
       
    Name                  & Type  & Value                          \\ \hline
    static1.squarespace.com. & CNAME  & prod.squarespace.map.fastly.net. \\ \hline
    % platform.linkedin.com & CNAME & 2-01-2c3e-0055.cdx.cedexis.net \\ \hline
    portfolio.adobe.com.  & CNAME & d.sni.global.fastly.net.        
   
        \end{tabular}
    \end{center}
\end{table}
